Thermal state structure in the Tavis--Cummings model and rapid simulations in mesoscopic quantum ensembles

Hybrid quantum systems consisting of a collection of N spin-1/2 particles uniformly interacting with an electromagnetic field, such as one confined in a cavity, are important for the development of quantum information processors and will be useful for metrology, as well as tests of collective behavior. Such systems are often modeled by the Tavis-Cummings model and having an accurate understanding of the thermal behaviors of this system is needed to understand the behavior of them in realistic environments. We quantitatively show in this work that the Dicke subspace approximation is at times invoked too readily, in specific we show that there is a temperature above which the degeneracies in the system become dominant and the Dicke subspace is minimally populated. This transition occurs at a lower temperature than priorly considered. When in such a temperature regime, the key constants of the motion are the total excitation count between the spin system and cavity and the collective angular momentum of the spin system. These enable perturbative expansions for thermal properties in terms of the energy shifts of dressed states, called Lamb shifts herein. These enable efficient numeric methods for obtaining certain parameters that scale as $O(\sqrt{N})$, and is thus highly efficient. These provide methods for approximating, and bounding, properties of these systems as well as characterizing the dominant population regions, including under perturbative noise. In the regime of stronger spin-spin coupling the perturbations outweigh the expansion series terms and inefficient methods likely are needed to be employed, removing the computational efficiency of simulating such systems. The results in this work can also be used for related systems such as coupled-cavity arrays, cavity mediated coupling of collective spin ensembles, and collective spin systems.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements} \label{sec:acknowledgements}

We thank... (for useful discussions etc)

\section*{Funding}
We gratefully thank the financial contributions of the Canada First Research Excellence Fund, Industry Canada, CERC (215284), NSERC (RGPIN-418579), CIFAR, the Province of Ontario, and Mike and Ophelia Lazaridis.

==> sections/dynamicsoverflow.tex <==

    
    \subsection{Dynamics with an Initially Thermal State}
    We have shown in this section the difficulty of cooling a Tavis--Cummings system to the Dicke subspace, where computations are tractable analytically. We now show that we can still make predictions for thermal states not contained solely within the Dicke subspace. 
    
    Consider an ensemble of identical spins, collectively coupled to a resonant single mode cavity, with a set of weakly coupled induction coils in the transverse plane. We assume that the coils are coupled identically to each spin, so that we induce collective control over the spin ensemble via the operators $\hat{J}_x$ and $\hat{J}_y$. The collective weak--coupling assumption ensures that the addition of the coils does not significantly perturb the energy eigenstructure. We define a ``Pulse and Measure'' experiment by the unitary pulse sequence,
    \begin{equation}
        \hat{U}(t) = \exp\big(-\ii t \H\big) \exp\big(-\ii \theta \hat{J}_x\big),
    \end{equation}
    and the observable of interest is
    \begin{equation}
        \avg{\hat{J}_x(t)} = \Tr\big(\hat{U}(t) \hat{\rho}_T \hat{U}(t)^\dagger \hat{J}_x \big). 
    \end{equation}
    If we restrict our analysis to a small flip--angle $\theta \ll 1$ and a small $N$, we can numerically produce the Fourier spectrum of this observable for low temperature samples in a closed system. We break this analysis into four steps: Determining the action of the small angle pulse on an energy eigenstate, finding the time evolution of the state, calculating the expectation value of the observable due to the evolution of the eigenstate, and finally averaging over the thermal state populations.
    
    Given an initial energy eigenstate,
    \begin{equation}
        \ket{\psi_E(0)} = \ket{E},
    \end{equation}
    we must compute 
    \begin{equation}
        \avg{\hat{J}_x(t)}_E = \matrixel{\psi_E(t)}{\hat{J}_x}{\psi_E(t)},
    \end{equation}
    where 
    \begin{equation}
        \ket{\psi_E(t)} = \hat{U}_p(t)\ket{\psi_E(0)}.
    \end{equation}
    We can make full use of the block diagonal representation of the Hamiltonian by similarly decomposing the $\theta$ pulse about the $x$-axis, using the following operator exponentiation formula \cite{curtright2014compact}: 
    \begin{equation}
        e^{-\ii \theta \hat{J}_x} = \bigoplus_{j}\bigg( \sum_{p=0}^{2j} \frac{c_p^j(\theta)}{p!}\big(-2 \ii \sin(\theta/2) \hat{J}_x)^p \bigg),
    \end{equation}
    where
    \begin{equation}
        c_p^j(\theta) = \bigg(\cos\frac{\theta}{2}\bigg)^\epsilon\underset{\floor{j-p/2}}{\operatorname{Trunc}}\bigg( \frac{\arcsin^p \sqrt{x}}{(\sqrt{x})^p(\sqrt{1-x})^\epsilon}\bigg),
    \end{equation}
    where $x=\sin^2(\theta/2)$ and $\epsilon =0.5(1-(-1)^{2j-p})$. With $\theta \ll 1$, we can approximate the action of the pulse unitary by restricting induced coherences to neighboring excitation subspaces of $\ket{E}$. That is, if $E = k\omega_0 + \lambda$, then we need only consider the subspaces with $k+1$ and $k-1$ excitations. Thus,
    \begin{equation}
        e^{-\ii \theta \hat{J}_x}\ket{E} =  \alpha_0 \ket{E} + \sum_q \alpha^+_q \ket{E^+_q} + \sum_r \alpha^-_r \ket{E^-_r},
    \end{equation}
    where it remains to compute the initial state coefficient $\alpha_0$, the $k+1$ excitation space coefficients $\alpha^+_q$, and the $k-1$ excitation space coefficients $\alpha^-_r$.
    
  Using the orthonormality of the energy eigenstates, we can write the coherences in terms of the matrix elements,
    \begin{align}
        \alpha_0 &= c_0^j(\theta),\\
        \alpha_q^\pm &= -2\ii \sin(\theta/2) c_1^j(\theta) \matrixel{E_q^\pm}{\hat{J}_x}{E}.
    \end{align}
    In the equations above, we truncated the series expansion for the pulse unitary by using the small angle approximation $\theta \ll 1$. In order to determine the explicit $\theta$ dependence of the prefactors of these matrix elements, we must consider the cases where $\epsilon = 0$ and $\epsilon = 1$, when $2j$ is even and odd, respectively. The small angle approximations have leading terms independent of $j$ and $\epsilon$, given by the following expressions,
    \begin{align}
        c_0^j(\theta) &= 1 + O(\theta^4),\\
        c_1^j(\theta) &= 1 + \frac{\theta^2}{24} + O(\theta^4).
    \end{align}
    
    In the energy eigenbasis,
    \begin{align}
        \nonumber \ket{\psi_E(t)}=\alpha_0 e^{-\ii E t } \ket{E} &+\sum_q \alpha^+_q e^{-\ii E^+_q t } \ket{E^+_q} \\
        &+ \sum_r \alpha^-_r e^{-\ii E^-_r t } \ket{E^-_r}.
    \end{align}
    Computing the expectation value of $\hat{J}_x$, we find
    \begin{align}
        \nonumber \avg{\hat{J}_x(t)}_E &= F(\theta) \bigg(\sum_q \abs{\matrixel{E_q^+}{\hat{J}_x}{E}}^2 \sin((E_q^+ - E) t)\\
        &+ \sum_r \abs{\matrixel{E_r^-}{\hat{J}_x}{E}}^2 \sin((E_r^- - E) t)\bigg), \\
        \nonumber \avg{\hat{J}_x(t)}_E &= \frac{F(\theta)}{2} \bigg(\sum_q \abs{\matrixel{E_q^+}{\hat{J}_+}{E}}^2 \sin((E_q^+ - E) t)\\
        &+ \sum_r \abs{\matrixel{E_r^-}{\hat{J}_-}{E}}^2 \sin((E_r^- - E) t)\bigg),
    \end{align}
    we find that the dependency of the FID signal on $\theta$ becomes an amplitude scaling factor given by
    \begin{equation}
        F(\theta) = -2\theta + O(\theta^5).
    \end{equation}
    Using linearity of expectation, we find the full thermal expectation value
    \begin{equation}
        \avg{\hat{J}_x(t)} = \sum_E P(E \ | \ \beta) \avg{\hat{J}_x(t)}_E.
    \end{equation}
     Given an initial energy eigenstate $\ket{E}$ in a $j,k$ subspace, we consider all states $\ket{E_f}$ in the $j,k-1$ and $j,k+1$ subspaces, each of which induce a delta--peak contribution to the spectrum located at a frequency of $\omega_{peak} = \pm(E_f - E)$, with amplitude of
    \begin{equation}
        A_{peak} = 2 \pi \abs{\theta} P(E \ | \ \beta) \abs{\matrixel{E_f}{\hat{J}_x}{E}}^2.
    \end{equation}
    
    Computing the FID spectrum is slower than computing a thermal state, as we need the eigenvectors in order to determine the matrix element of the peak amplitude. That being said, we can separate the $\hat{J}_+$ and $\hat{J}_-$ contributions, and compute the spectrum for particular values of $N$ and $T$. Utilizing the fact that angular dependency shows up as a global prefactor, we can divide the spectrum by $\theta$ in order to avoid recomputing the spectrum for select value of $\theta$. 
    
    % Picking the usual values of $N=100$, $\omega_0 = 10$ GHz, $g = 10$ Hz, with $T=120$ mK, we are able compute the FID spectrum. The results of these computations are given in figures \ref{fig:j_plus_contr} and \ref{fig:j_minus_contr}. 
    
    \begin{figure}[h!]
        \centering
        \includegraphics[scale = 0.35]{images/JxFermiSpectrum.png}
        \caption{Fourier spectrum of the observable $\avg{\hat{J}_+(t)}$. The horizontal axis is in units of $g_0$, shifted so that $\omega_0$ is located at the origin. The vertical axis is the peak amplitude, divided by $2\pi\theta$. For reference, $\omega_0 + g_0\sqrt{N}$ is located at 10 on the horizontal axis.}
        \label{fig:j_plus_contr}
    \end{figure}
    
    \begin{figure}[h!]
        \centering
        \includegraphics[scale = 0.35]{images/JxFermiSpectrum_counter.png}
        \caption{Fourier spectrum of the observable $\avg{\hat{J}_-(t)}$. The horizontal axis is in units of $g_0$, shifted so that $\omega_0$ is located at the origin. The vertical axis is the peak amplitude, divided by $2\pi\theta$. For reference, $\omega_0 + g_0\sqrt{N}$ is located at 10 on the horizontal axis.}
        \label{fig:j_minus_contr}
    \end{figure}
    
    The computation of the spectra illustrate that there are two dominant clustering of peaks, which at $T = 120$ mK are split about $\omega_0$ by a value less than $g\sqrt{N}$. We have illustrated that even though the thermal state does not appreciably populate the Dicke subspace at this temperature, we are still able to provide a precise calculation of the spectrum due to a pulse and measure experiment with small flip-angle.

==> sections/section01.tex <==
\section{Introduction} \label{sec:intro}
    In this paper, we focus on the collective interaction of an $N$ spin ensemble with a single mode quantum electromagnetic field. These systems have been used to verify quantum-ness of systems \cite{fink2008climbing} as well as useful tool for designing quantum devices and so a more full understanding of the thermal properties of these systems will aid further progress. In our system we take each particle to be non-interacting spin-1/2 particles, coupled uniformly to the electromagnetic field. After a rotating wave approximation, this is modeled by the  Tavis-Cummings (TC) Hamiltonian,
    
    \begin{equation}
        \H = \omega_c \hat{a}^\dagger \hat{a} + \omega_s \hat{J}_z + g_0(\hat{a}\hat{J}_+ + \hat{a}^\dagger \hat{J}_-),\label{eq.tc}
    \end{equation}
    where we work in natural units throughout this work ($\hbar=k_b=1$) \cite{tavis1968exact}.
    
    As mentioned in our previous work \cite{stasiuk2021generalized}, we have the ability to efficiently compute, as well as provide meaningful statistics on, the energy level structure of the Tavis-Cummings Hamiltonian under a certain set of assumptions. These assumptions can be realized in a laboratory setting, as we just require that the ensemble be on resonance with the cavity, $\omega_c = \omega_s \equiv \omega_0$, and that $g_0\sqrt{N} \ll \omega_0$ (albeit that this second expression is not quite correct as argued in our prior work \cite{stasiuk2021generalized}). Under these assumptions, we have that angular momentum, $j$, and the number of total excitations, $k$, that is excitations stored in both the spin ensemble and the cavity, are conserved. This induces a two parameter family of non-interacting subspaces.%, each with dimension less than or equal to $N+1$. The dimension is only equal to $N+1$ when $j=N/2$ and $k > N$.
    
    Throughout this paper we will assume that the spin-cavity system reached thermal equilibrium while coupled. This can be experimentally reproduced in an electron spin resonance (ESR) system with a superconducting strip, or with an ensemble of superconducting qubits all coupled to the same resonator.
    
    We begin with the definitions needed for our analysis. We then proceed to provide the uncoupled, $g_0=0$, partition function and average energy, which we then use to highlight the changes that occur from the introduction of the coupling between the spins and the cavity. Through this analysis we see that below a sufficiently small temperature the Dicke subspace is well populated, but beyond it the Dicke subspace is minimally populated and a perturbative approach must instead be used. We complement these mathematical results with numerical results which can show features that are overshadowed otherwise. These numerical results are achieved by implementing the improved computational methods from our prior work \cite{stasiuk2021generalized}.
    
    While we focus on the partition function and average energy of the system, the techniques employed and the results shown can be used for other thermodynamic properties such as Helmholtz free energy, entropy, and Gibbs free energy. Having access to both quick numerical methods for computing properties of these systems and perturbative expansions for these properties will allow additional insights into this model and hopefully for experimental setups.
    
    %We then focus on the main methodology of this paper, and showcase our ability to compute and visualize thermal states. Utilizing insights gained from the structure of the thermal state, we then detail our main results [which include x,y, and z--Lane]. The goal of this paper is two-fold: describe the thermal state of the TC Hamiltonian as a function of temperature, number of spins, and coupling strength.

==> sections/section02.tex <==
\section{Definitions} \label{sec:def}
    We include our notations and definitions in this section. The Pauli operators are written in the Zeeman basis, so that
    \begin{equation}
        \hat{\sigma}_z = \ketbra{\uparrow}{\uparrow} - \ketbra{\downarrow}{\downarrow},\quad 
        \hat{\sigma}_+ \ket{\downarrow} = \ket{\uparrow},\quad \hat{\sigma}_+ |\uparrow\rangle=0 .
    \end{equation}
    These spin operators can be combined as a sum of tensor products to produce the collective versions of these spin operators. Let $N$ be the number of spin--$1/2$ particles. Then the collective spin operators are given by
    \begin{equation}
        \hat{J}_z = \frac{1}{2} \sum_{i=1}^N \hat{\sigma}_z^{(i)},\quad
        \hat{J}_\pm = \sum_{i=1}^N \hat{\sigma}_\pm^{(i)}.
    \end{equation}
    where the superscript on the Pauli operator indicates action only on the $i$-th particle.
    
    %The collective operators span the $\mathfrak{sl}(2;\C)$ Lie algebra, and thus satisfy the following commutation relations:
    %\begin{equation}
    %    [\hat{J}_z , \hat{J}_\pm] = \pm \hat{J}_\pm,\quad
    %    [\hat{J}_+, \hat{J}_-] = 2\hat{J}_z.
    %\end{equation}
    \if{false}
    The collective operator algebra is a sub--algebra of self--adjoint operators acting on the $N$--spin system, and conveniently satisfies the same commutation relations as those for a single particle spin operator. By a change of basis, we can identify the transverse spin operators,
    \begin{align}
        \hat{J}_x &= \frac{1}{2}\big(\hat{J}_+ + \hat{J}_-\big),\\
        \hat{J}_y &= \frac{1}{2i}\big(\hat{J}_+ - \hat{J}_-\big).
    \end{align}
    The transverse spin operators, along with $\hat{J}_z$, span a collective $\mathfrak{su}(2)$ algebra, which differ from a single spin--1/2 Pauli operators in that the collective operators are not involutory. The representations of the $\mathfrak{sl}(2;\C)$ operators can be defined by their action on a state of total angular momentum $j$ with $z$ component $m$:\fi
    The action of these operators on a state of total angular momentum $j$ with $z$ component $m$ are given by:
    \begin{align}
        \hat{J}_z \ket{j,m} &= m\ket{j,m}\\
        \hat{J}_\pm \ket{j,m} &= \sqrt{j(j+1) - m(m\pm 1)}\ket{j,m \pm 1}.
    \end{align}
    
    We note that our Hamiltonian has two good quantum numbers representing conserved quantities. The first of these is the total angular momentum, $j$, which determines the eigenvalues of the total angular momentum operator, $\hat{\bm{J}}^2 = \hat{J}_x^2 + \hat{J}_y^2 + \hat{J}_z^2$, with eigenvalues $j(j+1)$. The second of these conserved quantities is the number of total excitations, $k$, given as the eigenvalues of the excitation operator,
    \begin{equation}
        \hat{K} = \hat{a}^\dagger\hat{a} + \hat{J}_z + \frac{N}{2}\openone.
    \end{equation}
    The scaled identity term in the excitation operator ensures excitations are non--negative, as the action of $\hat{J}_z$ on the ground state has eigenvalue $-N/2$.
    \if{false}
    All of the Hamiltonians considered in this work share the same internal structure, defined by 
    \begin{equation}
        \H_0 =  \omega_0 (\hat{a}^\dagger\hat{a} + \hat{J}_z).
    \end{equation}
    The interaction Hamiltonian is given by the Dicke model \cite{dicke1954coherence}:
    \begin{equation}\label{dicke}
        \H_{D,int} = 2g_0 \big(\hat{a} + \hat{a}^\dagger\big) \hat{J}_x.
    \end{equation}
    Applying the rotating wave approximation, the counter--rotating term is discarded, leaving us with
    \begin{equation}
        \H_{int} = g_0 \big(\hat{a} \hat{J}_+ + \hat{a}^\dagger \hat{J}_- \big),
    \end{equation}
    which is the interaction term in the Tavis--Cummings (TC) Hamiltonian. \if{false}Note that tensor products are omitted for brevity, so that, for example,
    \begin{equation}
        \hat{a} \otimes \hat{J}_+ \equiv \hat{a}\hat{J}_+.
    \end{equation}\fi

    Lastly, we note that all states live within the Hilbert space,
    \begin{equation}
        \mathscr{H} = \operatorname{L}^2\left(\mathbb{R}\right) \otimes \big(\C^2\big)^{\otimes N}.
    \end{equation}
    \fi

We recall next the pertinent aspects and definitions from our prior work. Our Hamiltonian may be written in direct sum form as
    \begin{equation}
        \H \cong \bigoplus_{j,k}\big( \omega_0 k \openone_{j,k} +  g_0 L(j,k)\big),
    \end{equation}
where $L(j,k)$ are hollow tridiagonal square matrices with known entries and dimension $|\mathcal{B}_{j,k}|=\min\{2j+1,k-k_0(j)+1\}$, where $k_0(j)=N/2-j$. The set of eigenvalues for $L(j,k)$ is written as $\Lambda(j,k)$. \if{false} interaction Hamiltonian, which we define in equation \eqref{eq:coupling_matrix} and refer to as the coupling matrices. 
    
We define a basis for a general $(j,k)$ subspace with total angular momentum $j$ and $k$ excitations as 
    \begin{equation}\label{eq:lamb_basis}
        \mathcal{B}_{j,k} = \lbrace \ket{\alpha_{j,k}} \,|\, \alpha = 1,\cdots,n_{j,k}, n_{j,k} + 1\rbrace,
    \end{equation}
    using a shorthand ket representation of the tensor product of a spin-cavity state
    \begin{equation}
        \ket{\alpha_{j,k}} = \ket{k-\alpha-k_0(j)}\ket{j,-j+\alpha}.
    \end{equation}
    The single parameter, $\alpha$, provides a convenient representation of states within a $(j,k)$ subspace. The value, $n_{j,k} = \abs{ \mathcal{B}_{j,k} } - 1$, one less than the dimension, is chosen for convenience. We define $k_0(j) = N/2-j$ as the number of excitations present in the ground state of an angular momentum $j$ subspace within an $N$ spin ensemble. Explicitly, $n_{j,k}$ is given as
    \begin{equation}
        n_{j,k} = \operatorname{min}\lbrace 2j, k - k_0(j)\rbrace.
    \end{equation}
    If $k < k_0(j)$, then the basis set is empty and there are no states present at this excitation level within the $j$ angular momentum subspace.

    \if{false}The coupling matrices' entries can be found by applying the interaction term from $\mathcal{\hat{H}}_{TC}$ on the bases defined in equation \eqref{eq:lamb_basis}. \fi The Lamb shift coupling matrix for the $(j,k)$ subspace is then given by
    \begin{align}\label{eq:coupling_matrix}
        \nonumber L(j,k) &= \sum_{\alpha=1}^{n_{j,k}} l_{\alpha}(j,k)\bigg(\ketbra{\alpha_{j,k}}{(\alpha+1)_{j,k}}\\
        &\hspace{1.5cm}+ \ketbra{(\alpha+1)_{j,k}}{\alpha_{j,k}}\bigg),
    \end{align}
    where the matrix elements $l_{\alpha}(j,k)$ are given by
    \begin{align}
        \nonumber &\frac{1}{ g_0}\matrixel{\alpha_{j,k}}{\H_{int}}{(\alpha+1)_{j,k}}\\
        &= \sqrt{\big(2\alpha j - \alpha(\alpha-1)
        \big)\big(k-k_0(j)-\alpha+1\big)}.
    \end{align}
    In the above expression subscripts are only included within kets such as $\ket{\alpha_{j,k}}$, while $\alpha$ itself is a scalar.\fi
    
    The index $j$ runs from $N/2$ to $0$ ($1/2$) when $N$ is even (odd). Each angular momentum space is of dimension $2j+1$. The degeneracy of the subspace with total angular momentum $j$ on $N$ spins is given as
    \begin{equation}
        d_j = \frac{N! (2j+1)}{(N/2 - j)!(N/2+j+1)!}.
    \end{equation}
    That is, there are $d_j$ disjoint angular momentum subspaces with total angular momentum $j$ present in a direct sum decomposition of $\big(\C^2\big)^{\otimes N}$ \cite{wesenberg2002mixed}.
    
    The eigenvalues for one of these coupling matrices may be computed in $O(|\mathcal{B}_{j,k}|\log |\mathcal{B}_{j,k}|)$, while the sum is always zero, and the second moment has an analytic expression. \if{false}The eigenvectors take $O(|\mathcal{B}_{j,k}|^2)$.\fi Lastly, the degeneracies have a region of strong support of $O(\sqrt{N})$ about $j^*$, the most degenerate angular momentum subspace, where $j^*\approx \sqrt{N}/2$. These observations aide in both our mathematical analysis and our numerical results.
    
    %The computational advantage over a naive full Hamiltonian diagonalization is further compounded, given that the structure of the Hamiltonian is dominated by the lowest $O(\sqrt{N})$ angular momentum subspaces out of the total $N$ distinct angular momentum subspaces. We will show that an efficient calculation of the structure of the Hamiltonian can be utilized to provided insight into the structure of the thermal states of this Hamiltonian.

==> sections/section03.tex <==
\section{Results} \label{sec:methods}
    In the Tavis--Cummings model we usually find ourselves restricting to the Dicke subspace, so that we can find analytical and tractable numerical solutions to the functions of interest. However, these methods often fail to accurately represent the states and dynamics of the model, especially when the Dicke subspace is not sufficiently populated, as we have shown in our previous work \cite{stasiuk2021generalized}. A common approximation procedure is the semi--classical approximation, which we have included in the appendix for completeness.
    
    In this work we are interested in the thermal states of the Tavis--Cummings model compared to the case where the cavity and spin ensemble are non--interacting. We begin by providing the behaviors of the non--interacting model and will proceed to the more general Tavis--Cummings case. The cavity and spin ensembles are said to be non--interacting if the coupling strength $g_0$ is zero or if the spin and cavity are sufficiently out of resonance. So that this case more closely matches that of the interacting Tavis--Cummings model we will assume that the coupling strength $g_0$ is zero.
    
    The thermal state of the spin ensemble is given by
    \begin{eqnarray}
         \hat{\rho}_{\text{th}}^{\text{spins}} &=& \otimes_{i=1}^N \frac{e^{-\beta \omega_0/2}|\uparrow\rangle\langle\uparrow|+e^{\beta\omega_0/2}|\downarrow\rangle\langle\downarrow|}{e^{-\beta \omega_0/2}+e^{\beta\omega_0/2}} \\
        &=& \otimes_{i=1}^N \frac{1}{2}\bigg(\openone - \tanh\big(\frac{\beta \omega_0}{2}\big) \hat{\sigma}_z^{(i)}\bigg). %I've verified this equation for sanity sake, the prior line is to make it clearer where it comes from
        %\nonumber &= \frac{1}{2^N}\bigg( \openone - \tanh\big(\frac{\beta\omega_0}{2}\big) \sum_{i=1}^N \hat{\sigma}_z^{(i)} \\
        %&\hspace{.75cm} + \tanh^2\big(\frac{\beta\omega_0}{2}\big) \sum_{i\neq j}^N \hat{\sigma}_z^{(i)}\hat{\sigma}_z^{(j)} - \cdots\bigg).
    \end{eqnarray}
    The thermal state of a cavity system is given by
    \begin{equation}
        \hat{\rho}_{\text{th}}^{\text{cavity}} = \big(1-e^{-\beta\omega_0}\big)\sum_{k=0}^{\infty}e^{-k \beta \omega_0}\ketbra{k}{k}.
    \end{equation}
    
    As there is no coupling term being considered at this time the thermal state of the two systems, having thermalized separately, is given by the product state
        $\hat{\rho} = \hat{\rho}_{\text{th}}^{\text{c}} \otimes \hat{\rho}_{\text{th}}^{\text{s}}$,
    %For $g>0$ and $\omega_s = \omega_c$, the situation is more complex due to the interaction term which creates entanglement between the spins and the cavity in the energy eigenbasis \cite{}. This coupling prohibits writing the thermal state of the joint system as a product state over the subsystems, as we have done above. We will describe thermal states of this coupled model by working in the energy eigenbasis of the Hamiltonian. Determining the energy eigensystem presents its own challenges, but by utilizing symmetry we have previously shown vast improvements to the efficiency of computing this structure \cite{ourpriorwork}. 
    so the partition function of this joint system can then be given as:
    \begin{equation}\label{z0}
        Z_0=(1-e^{-\beta\omega_0})^{-1}(e^{-\beta\omega_0/2}+e^{\beta\omega_0/2})^N.
    \end{equation}
    We also provide the average energy of this system as we will compare this to that of the coupled Tavis--Cummings model:
    \begin{equation}
        \langle E\rangle_{0}=\omega_0 (e^{\beta \omega_0}-1)^{-1}+\frac{\omega_0 N}{2}\left(1 - \tanh\left(\frac{\beta \omega_0}{2}\right)\right).
    \end{equation}
    This has a limit of $0$ at $T=0$, as we have shifted the Zeeman term by $\frac{N}{2}\openone$, and a high temperature limit of:
    %\begin{equation}
    %    \beta^{-1}-\frac{\omega_0}{2}+\frac{\beta\omega_0^2}{12}+\frac{\omega_0 N}{2}(1-\frac{\beta\omega_0}{2})+O(\beta^3)
    %\end{equation}
    \begin{equation}
        T+\frac{\omega_0}{2}(N-1)-\frac{\omega_0^2}{4}(N-\frac{1}{3})T^{-1}+O(T^{-3}).
    \end{equation}
    Having discussed the $g_0=0$ case, we are now prepared to make remarks about the $g_0> 0$ case.
    
    \subsection{Quasicritical temperature and low temperature information}
    
    STATE SUPER CLEARLY TEMP RANGE
    
    We begin by remarking on the comparative simplicity of the very low-temperature regime for this problem. Due to the utility of the analytic calculations in the Dicke subspace, it is useful to have a temperature dependent condition for determining whether the system is well approximated by a restriction to the Dicke subspace. Notably, since angular momentum is a conserved quantity when restricting to collective operators, any population that starts outside of the Dicke subspace cannot be transferred into it by collective dynamics. This has made the analysis of cavity cooling quite difficult, as one needs to break the collective symmetry in order to cool to the Dicke ground state \cite{wood2014cavity, wood2016cavity}. Further, as we have shown in figure \ref{fig:thermal_distro}, the thermal distributions indicate that we require the system to thermalize with an environment described by temperatures on the order of tens of mK or lower in order to appreciably populate the Dicke subspace.
    
    Using the block diagonal structure of the Hamiltonian we may write the partition function as:
    \begin{equation}
        Z_{total}(\beta) = \sum_{k=0}^\infty \sum_{j=j_0(k)}^{N/2}\bigg( d_j e^{-\beta k \omega_0} \sum_{\lambda\in\Lambda(j,k)} e^{-\beta \lambda g}\bigg),
    \end{equation}
    where we have defined
    \begin{equation}
        j_0(k) = \max \lbrace N/2-k, \ N/2 - \floor{N/2}\rbrace.
    \end{equation}
    For low temperatures, the degeneracy, $d_j$ plays an extremely important role within the partition function. We find a quasicritical temperature in our system, with value roughly $T_c=\omega_0/\log N$ (see appendix). Below $T_c$ a fair portion of the population is contained in the lowest lying energy states with the largest collective angular momentum, such as the Dicke subspace, but once we are above $T_c$ the rapid degeneracy increase across angular momentum subspaces dominates and the population is strongly biased toward the available angular momentum space closest to $j^*$.
    
    %Focus on showing that Dicke approximation is bad. Show relative population levels. Is picture enough? It doesn't feel like quite enough. I want a simple truncated series that proves that Dicke is empty--Dicke and neighbor, first few levels, and find $T$ such that Dicke is $\leq \frac{1}{2}$.
    
    \subsection{Higher Temperature Perturbative Expansions}
    
    We now turn our attention to the case of higher temperatures. We find that we may expand the partition function in a perturbative series expansion. So long as $T\gtrsim g_0N\sqrt{\kappa}$, where $\kappa$ is the largest excitation with non-negligible population, (or generally $\beta\omega_0<1$, which is around $0.8$ Kelvin for a typical value of $\omega_0$), we may approximate $Z_{total}(\beta)\approx Z_0(\beta)+Z_{pert}(\beta)$ with:
    \begin{equation}
        Z_0(\beta)=\sum_k e^{-\beta k\omega}\sum_j d_j|\mathcal{B}_{j,k}|
    \end{equation}
    which is the same as equation (\ref{z0}), and
    \begin{equation}
        Z_{pert}(\beta)\approx \frac{(\beta g_0)^2}{2}\sum_k e^{-\beta k\omega}\sum_j d_j|\mathcal{B}_{j,k}| Var(\Lambda(j,k)).
    \end{equation}
    This then leads to the following expression for the average energy in this system:
    \begin{equation}
        \langle E\rangle\approx \langle k\rangle _{Z_0}\omega_0+((\langle k\rangle_{Z_{pert}}-\langle k\rangle_{Z_0}) \omega_0-\frac{2}{\beta})\frac{Z_{pert}}{Z_0}.
    \end{equation}
    Alternatively we can express this in terms of the change in the average energy of our spin-cavity system:
    \begin{equation}
        \Delta\langle E\rangle =((\langle k\rangle_{Z_{pert}}-\langle k\rangle_{Z_0}) \omega_0-\frac{2}{\beta})\frac{Z_{pert}}{Z_0},
    \end{equation}
    where $\langle k\rangle_{Z_0}$ is the average number of excitations with respect to the distribution $Z_0(\beta,k)/Z_0$, and $\langle k\rangle_{Z_{pert}}$ is the analogous expectation over the perturbative partition function. Additionally, we have as the shift induced in the Helmholtz free energy:
    \begin{equation}
        \Delta \langle A\rangle=\frac{Z_{pert}}{Z_0}
    \end{equation}
    
    \subsection{Computational Improvements}
     We note that the computational complexity of computing the first order correction is faster than the next order as we have an analytic expression for $Var(\Lambda(j,k))$--computing the first order correction costs $O(NT)$. Including the next term would cost $O(N^2T)$ (although this cost expression would not increase if another order or two were included as well), however, for machine precision level $O(N^2 T\log N)$ time is needed. If, however, we also utilize our knowledge that the degeneracies have a relatively small region of strong support with size $O(\sqrt{N})$, these time complexities reduce to: $O(\sqrt{N} T)$, $O(NT)$, and $O(N^{3/2}T\log N)$, respectively, where the extra half power for the last one comes from having to solve matrices of size up to $N\times N$. Note that in all the prior expressions we have suppressed the dependency on $\omega_0$ as this is just a scaling of the variable $T$ in effect. As thermodynamic properties are computed using the partition function and this is the bottle neck for performing those computations, most thermodynamic functions should take the same run time.
     
     Beyond these numerical speedups, we may make two general remarks on $\Delta\langle E\rangle$. Firstly, as $g_0$ tends toward zero, so does this expression. Secondly, as $\langle k\rangle_{Z_{pert}}<\langle k\rangle_{Z_0}$ [due to it being a higher moment of an exponential distribution], $\Delta \langle E\rangle\leq 0$, meaning that the introduction of the coupling reduces the average energy in system. Further simplifications of the expression for $\Delta\langle E\rangle$ are beyond the scope of this work, however, we provide some illustrative figures as well as analysis in the next subsection.
     \begin{widetext}
     \begin{center}
\begin{tabular}{||c| c| c| c| c||} 
 \hline
 Error & $O(g_0^4)$ & $O(g_0^{2c}),\ c> 2$ & Machine Precision & Naive \\ [0.5ex] 
 \hline\hline
 $Z_{pert}$, $Z_{tot}$, $\Delta\langle A\rangle$, $\Delta \langle E\rangle$ & $O(T\sqrt{N})$ & $O(NT)$ & $O(TN\log N)$ & $O(TN^3)$ \\ 
 \hline
 $\mathcal{O}(j,k)$ (no region of strong support promise) & $O(NT)$ & $O(N^2T)$ & $O(TN^2\log N)$ & $O(TN^3)$ \\
 \hline
 $\mathcal{O}(j,k)$ (region of strong support promised) & $O(T\sqrt{N})$ & $O(NT)$ & $O(TN\log N)$ & $O(TN^3)$ \\ [1ex]
 \hline
\end{tabular}
\end{center}
 \end{widetext}   
    \subsection{Numerical Computation of the Thermal Distribution}
    While the expressions in the previous sections provided some insights, they also caused other aspects to be overshadowed. Here we describe how we compute the thermal distribution, instead of the partition function, as well as the energy shift induced from the coupling $\Delta\langle E\rangle$.
    
    By decomposing the TC system into subspaces labeled by angular momentum $j$ and excitations $k$, we can efficiently solve for the energy eigenvalues. We can write the thermal state populations as a probability distribution over the allowed energy levels of the system. That is, we determine the set,
    \begin{equation}
        \mathcal{E}(\beta) = \lbrace (E, P(E \ | \ \beta)) \,|\, \forall E, \H \ket{E} = E \ket{E} \rbrace,
    \end{equation}
    where the probability of the label $E$ is determined by the number of eigenstates with energy $E$, given by $d(E)$, and the temperature of the system:
    \begin{equation}
        P(E \ | \ \beta) = d(E) e^{-\beta E} / Z(\beta).
    \end{equation}
    
    We find that the eigenvalue problem needs to only be solved once for a given value of $N$ and by storing the energy spectrum we can efficiently compute the distribution of the thermal state for a given new temperature or temperature range. The results are shown in figure \ref{fig:thermal_distro}.

    \begin{figure}[h!]
    
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=.95\linewidth]{images/point025_kelvin.png}
        \caption{$T = 0.025$ K}
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=.95\linewidth]{images/point2_kelvin.png}
        \caption{$T = 0.200$ K}
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \includegraphics[width=.95\linewidth]{images/1_kelvin.png}
        \caption{$T = 1.000$ K}
        \label{fig:1c}
    \end{subfigure}
    
    \caption{Thermal population distribution for the TC Hamiltonian at $\omega_0 = 10$ GHz, $g_0 = 10$ Hz, and $N=100$ spins, for selected temperatures of $T=0.025,0.200,1.000$ Kelvin. Notice that at each temperature, the ground state population is not appreciably populated for temperatures on the order of hundreds of mK or greater.}
    \label{fig:thermal_distro}

    \end{figure}

   To demonstrate this numerically, we consider the parameters $\omega_0 = 10$ GHz, $g_0 = 10$ Hz, and temperatures at or less than $1$ Kelvin. These parameters can be feasibly realized in an ESR system \cite{}. We demonstrate our ability to determine the thermal distribution by particularizing to $N=100$ identical spin--1/2 particles.

    It may be somewhat surprising to see that temperatures near $200$ mK result in a fairly high energy distribution, populating subspaces with 30 to 60 excitations. Even in the case of $25$ mK, it appears that the system has not fully cooled to its ground state.% Later in this work we revisit the distribution of population at a given temperature and showcase the relative impact of the Boltzmann factor, $e^{-\beta \omega_0}$, and the degeneracies of angular momentum subspaces, $d_j$, on the distribution of population in a thermal state.
    
    Plot for $\Delta\langle E\rangle$ instead! I want a plot of this!!! One curve with and one without, as well as just a plot of it.
    
\if{false}    We can further investigate the interplay of $N$ and $T$ by determining the average energy of the system. The average energy of the system is given by: 
    \begin{equation}
    \avg{E}(N, \ T) = \sum_{E} P(E \ | \ \beta) E.
    \end{equation}
    This summation for the average energy showcases that for a given $N$, the average energy can be quickly computed using the cached energy eigenstructure computed earlier. [what is the runtime of this? I feel like it's still $O(NT)$ or larger...] We plot the average energy as a function of temperature for select values of $N$.
    
    \begin{figure*}[h!]
    \begin{subfigure}{.33\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{images/lowtemp_avgE.png}
        \caption{Average energy as a function of temperature. Cooling the system to the ground state would require that the average energy drops below the one excitation mark, which is below $20$ mK for $N>100$. $\omega_0 = 10$ GHz, $g = 10$ Hz.}
        \label{fig:2a}

    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
        \includegraphics[width=.95\linewidth]{images/hightemp_avgE.png}
        \caption{Average energy as a function of temperature. Cooling the system to the ground state would require that the average energy drops below the one excitation mark, which is below $20$ mK for $N>100$. $\omega_0 = 10$ GHz, $g = 10$ Hz.}
        \label{fig:2b}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{images/lowtemp_avgE_funcN.png}
        \caption{Demonstration of the linearity of the average energy as a function of the number of spins, $N$, at select values of constant temperature. $\omega_0 = 10$ GHz, $g = 10$ Hz.}
        \label{fig:2c}
    \end{subfigure}
    \end{figure*}

    
    Figure \ref{fig:2c} illustrates that as temperature increases from 0 Kelvin, the average energy rapidly increases, with larger values of $N$ leading to a faster departure from the ground state. Based on the distributions in figure 1(a)-(c), we do not expect the average thermal energy to be highly sensitivity to temperature over the entire domain. This is confirmed in figure \ref{fig:2a}.
    
    \fi
    %Qualitatively, figure \ref{fig:hightemp_avgE} shows us that the average energy as a function of temperature has a concavity change. At the lower temperatures, we have a region of positive concavity, indicating a rapid departure from the ground state of the system with increasing temperature. As the temperature continues to increase, the concavity changes to a negative value, leading to a slowing of the rate at which the average energy increases with temperature.
    
\if{false}    From figures \ref{fig:2a} and \ref{fig:2b}, it appears that the average energy as a function of $N$ at a fixed temperature is given by a linear function. This suspicion is confirmed in figure \ref{fig:2c}. The linear dependence of the average energy as a function of $N$ persists through all tested values of $N$ and $T$, with $r^2 = 1$ to within machine precision. This leads to the following relationship,
    \begin{equation}
        \avg{E}(N,T) = m(T) N + b(T),
    \end{equation}
    where $m(T)$ and $b(T)$ are undetermined functions of temperature.
    
    The linearity of the average energy as a function of $N$ hints at the fact that cooling the TC model to the ground state requires increasingly lower temperatures as the number of spins increases. \if{false} As a direct comparison, we can compute the average energy of an ensemble of $N$ identical spins with identical Zeeman shifts. With an energy shifted Hamiltonian of 
    \begin{equation}
        \H_s = \omega_0\bigg( \hat{J}_z + \frac{N}{2}\openone\bigg),
    \end{equation}
    we can immediately determine the average energy:
    \begin{equation}
        \avg{E}_s(N,T) = \frac{\omega_0 N}{2}\bigg(1 - \tanh\left(\frac{\beta \omega_0}{2}\right)\bigg).
    \end{equation}
    Due to the energy level shift in the Hamiltonian, to count the number of excitations, the high temperature limit of this function corresponds to $N/2$ excitations, with an underlying thermal state given by the fully mixed state.  
    
    Similarly, the average energy of the quantized EM field with an uncoupled Hamiltonian of
    \begin{equation}
        \H_c = \omega_0 \hat{a}^\dagger \hat{a},
    \end{equation}
    is computed such that
    \begin{equation}
        \avg{E}_c(T) = \omega_0 \frac{e^{-\beta \omega_0}}{1-e^{-\beta\omega_0}}.
    \end{equation}
    The low temperature limit of this function is 0 as expected, but the high temperature limit is a little harder to see. Expanding about $\beta = 0$, and transforming to $T$, we find
    \begin{equation}
        \avg{E}_c(T) = k_B T - \frac{\omega_0}{2} + \frac{\omega_0^2}{12 k_B T} + O(1/T^2).
    \end{equation}
    Thus we expect linearly increasing energy with temperature in the high temperature limit.
    \fi
    
    
 A linear regression determines the approximate functional form of $m(T)$ and $b(T)$, but its predictive capabilities are limited, and errors in $m(T)$ become magnified by the prefactor of $N$. We continue to work with $\omega_0 = 10$ GHz, $g = 10$ Hz as our choice of parameters for the regression step of the analysis. Under the fixed parameters, we applied linear regression to each set of constant temperature. Using non--linear regression on the set of slopes and intercepts we find:
    
    \begin{align}
        m(T) &\approx \exp\bigg(\frac{0.0435}{T^{1.1}}-0.688\bigg)T^{-0.02276}, \text{ and}\\
        b(T) &\approx  T \exp\bigg(2.57011 - \frac{0.03675}{T}\bigg).
    \end{align}

    Qualitatively, it appears that we can attribute the main features of these functions to the underlying subsystems. The slope as a function of temperature, $m(T)$, decays to 0 as $T\longrightarrow\infty$ and has its contribution to the average energy magnified by the size of the spin ensemble. Thus, $m(T)$ is the spin dominant contribution to the average energy. Furthermore, we see that for large $T$, $b(T)$ is strongly dominated by a linear growth in average energy, which implies that $b(T)$ is a dominated by photonic contributions. One could expand this regression analysis into a multi--parameter model to capture the dependence of the expected energy on $\omega_0$ and $g_0$.
    
    \fi
    
    We see that while the existence of the coupling terms inhibits our ability to determine analytic solutions for the thermal state of the TC model, we find that we can still draw strong parallels on its behavior to the underlying subsystems. This concept is possibly best illustrated in figure \ref{fig:1c}, where the thermal distribution has two peaks, indicating that temperatures near 1 K form an intermediate regime, dominated by neither spin contributions, nor photonic contributions.
    
%    [broadly, the energy is determined by the same relationship due to the non-interacting portion of the Hamiltonian. I would rather have information on the shape of the perturbation to the energy. I worry that this current regression form follows trivially...--Lane]

==> sections/section04.tex <==
\section{Results} \label{sec:results}

%    In this section, we make use of our ability to determine thermal states of the Tavis--Cummings Hamiltonian to provide a variety of new insights. We begin with determining a ground state cut--off temperature, above which the Dicke ground state is not appreciably occupied. With experiments in mind, we describe a small flip--angle pulse and measure experiment.


==> sections/section05.tex <==
\section{Discussion} \label{sec:discussion}
    
    
    
    
    

==> sections/section06.tex <==
\section{Conclusion} \label{sec:conclusion}
    
   % In this paper, we have illustrated some of the potential applications of an efficiently calculable eigenstructure for the Tavis--Cummings Hamiltonian. With knowledge of the energy eigenvalues, we can map out the thermal landscape numerically, providing experimental researchers the necessary tools to determine where state population is at a given temperature. Further, we can provide a benchmark temperature for cooling in order to appreciably populate the Dicke ground state. Notably, this cutoff temperature is much colder than perhaps previously expected \cite{}.
    
%    All is not lost if the Dicke subspace does not contain a majority of the state population, as we have illustrated that we can still make precise predictions of experimental spectra for a sample where the Dicke subspace is not appreciably populated. This procedure works best with smaller sized spin ensembles, and thus lends itself well to superconducting qubit ensembles, as it may be difficult to isolate $100$ electron spins for an ESR sample.
    
 %   The algorithms used to calculate the spectrum shown in figures \ref{fig:j_plus_contr} and \ref{fig:j_minus_contr} are relatively naive, and there is room to improve their efficiency, both in time and in memory. The progress towards numerically predicting spin ensembles on the order of $N=10^{12}$ spins will likely be outpaced by theoretical tools designed to solely predict the features of interest, as opposed to predicting every frequency component across entire spectrum.
 
    In this work we have described the thermal state for the Tavis--Cummings model, as well as provided a technique for perturbatively computing various thermal properties, as well as improvements to numerical methods. While these are useful aspects to know, converting these properties into other observables such as a free-induction decay (FID) would aid in verifying these results. In addition, this work assumes that the spin-cavity system is a closed system. Thus, while we allow thermalization with a reference bath, we do not allow for this interaction to induce any dissipation operators on the spins or the cavity. In a real experimental setting, there are a variety of noise sources which will inevitably break some of our idealizations and understanding how these will impact observations is crucial. For instance, a direct consequence will be that the computed Fourier spectrum of the FID will be composed not of a sum of delta functions, but rather, a sum of broadened curves. A full open quantum system treatment would be needed in order to properly predict the spectrum in this setting, which leads to new challenges, but also greater utility of these systems.
